Q-Turn: Changing Paradigms In Quantum Science

Quantum information is a rapidly-growing interdisciplinary field at the intersection of information science, computer science, mathematics, philosophy, and quantum science, working at the core of our quantum technologies. Regardless of its scientific success, quantum information is not exempt from the intrinsic features that come from the fact that scientists are humans and members of society: both the good and the bad of our social practices leak into the scientific activity. In our scientific community, diversity and equal opportunity problems are particularly difficult to observe due to social, economic, or cultural barriers, often remaining invisible. How can our lack of awareness negatively influence the progress of science in the long term? How can our community grow into a better version of itself? This article reflects on how research events - such as conferences - can contribute to a shift in our culture. This reflection draws on what we learn from Q-Turn: an initiative triggered by postdoctoral researchers to discuss these questions. One of Q-turn's main missions is to foster an inclusive community and highlight outstanding research that may be under-appreciated in other high-impact venues due to systemic biases. As well as a scientific program, Q-turn features talks and discussions on issues that affect the quantum information community, ranging from diversity and inclusion, health and mental health, to workers' rights. In this perspective article, we will consider Q-Turn as an example of how a research community can work to tackle systematic biases, review the successes, and identify further points for development.

==> tikzlibrarypie.code.tex <==
% SPDX-License-Identifier: GPL-2.0-only OR LPPL-1.3c
\RequirePackage{scalefnt}

%
% Utilities
%

\def\pgfpie@ifx#1#2{%
  \ifx#1#2%
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifdim#1#2#3{%
  \ifdim\dimexpr#1\relax#2\dimexpr#3\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifnum#1#2#3{%
  \ifnum\numexpr#1\relax#2\numexpr#3\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifodd#1{%
  \ifodd\numexpr#1\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@newif#1{%
  \csname newif\expandafter\endcsname\csname ifpgfpie@#1\endcsname
  \expandafter\def\csname pgfpie@if#1\expandafter\endcsname\expandafter{%
    \csname ifpgfpie@#1\endcsname
      \expandafter\pgfutil@firstoftwo
    \else
      \expandafter\pgfutil@secondoftwo
    \fi}%
}

%
% Constants for text comparison
%

\def\pgfpie@text@inside{inside}
\def\pgfpie@text@legend{legend}
\def\pgfpie@sum@c{100}
\def\pgfpie@sum@auto{auto}

% args:
% #1: begin angle
% #2: end angle
% #3: number
% #4: label
% #5: explode
% #6: fill color
% #7: radius
% #8: center
\def\pgfpie@slice#1#2#3#4#5#6#7#8{%
  \pgfmathparse{0.5*(#1)+0.5*(#2)}
  \let\pgfpie@midangle\pgfmathresult

  \path (#8) -- ++({\pgfpie@midangle}:{#5}) coordinate (pgfpie@O);

  \pgfmathparse{(#7)+(#5)}
  \let\pgfpie@radius\pgfmathresult
  
  % slice
  \draw[line join=round,fill={#6},\pgfpie@style] (pgfpie@O) -- ++({#1}:{#7}) arc ({#1}:{#2}:{#7}) -- cycle;

  \pgfpie@ifchangedirection{%
    \pgfmathparse{min(((#1)-(#2)-10)/110*(-0.3),0)}
  }{%
    \pgfmathparse{min(((#2)-(#1)-10)/110*(-0.3),0)}
  }%
  
  \pgfmathparse{(max(\pgfmathresult,-0.5) + 0.8)*(#7)}
  \let\pgfpie@innerpos\pgfmathresult

  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    % label and number together
    \path (pgfpie@O) -- ++({\pgfpie@midangle}:{\pgfpie@innerpos}) node[align=center]
    {\pgfpie@scalefont{#3}\pgfpie@labeltext{#4}\\\pgfpie@numbertext{#3}};
  }{%
    % label
    \pgfpie@ifhidelabel{}{%
      \pgfpie@iflegend{}{%
        \path (pgfpie@O) -- ++ ({\pgfpie@midangle}:{\pgfpie@radius})
        node[inner sep=0, \pgfpie@text={\pgfpie@midangle:#4}]{};
      }%
    }%

    % number
    \path (pgfpie@O) -- ++({\pgfpie@midangle}:{\pgfpie@innerpos}) node
    {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}};
  }%
}

\def\pgfpie@findColor#1{%
  \pgfmathparse{int(mod(#1,\the\pgfpie@colorLength))}%
  \let\pgfpie@ci\pgfmathresult
  \foreach \pgfpie@c [count=\pgfpie@j from 0] in \pgfpie@color {%
    \pgfpie@ifnum{\pgfpie@j}{=}{\pgfpie@ci}{%
      \xdef\pgfpie@thecolor{\pgfpie@c}%
      \breakforeach
    }{}%
  }
}

\def\pgfpie@findExplode#1{%
  \pgfmathparse{int(mod(#1,\the\pgfpie@explodeLength))}%
  \let\pgfpie@ei\pgfmathresult
  \foreach \pgfpie@e [count=\pgfpie@j from 0] in \pgfpie@explode {%
    \pgfpie@ifnum{\pgfpie@j}{=}{\pgfpie@ei}{%
      \xdef\pgfpie@theexplode{\pgfpie@e}%
      \breakforeach
    }{}%
  }%
}

% #1: bottom left point
% #2: size
% #3: number
% #4: color
% #5: text
\def\pgfpie@square#1#2#3#4#5{%
  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    \draw[fill={#4},\pgfpie@style] (#1) rectangle node[align=center]
    {\pgfpie@scalefont{#3}\pgfpie@labeltext{#5}\\\pgfpie@numbertext{#3}} ++(#2);
  }{%
    \draw[fill={#4},\pgfpie@style] (#1) rectangle node
    {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}} ++(#2);
  }%
}

% #1: pos
% #2: radius
% #3: number
% #4: color
% $5: style
% $6: label
\def\pgfpie@cloud#1#2#3#4#5#6{%
  \draw[fill=#4, #5] (#1) circle[radius=#2];
  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    \node[align=center] at (#1) {\pgfpie@scalefont{#3}\pgfpie@labeltext{#6}\\\pgfpie@numbertext{#3}};
  }{%
    \node at (#1) {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}};
  }%
}

\newdimen\pgfpie@angleEnd
\newcount\pgfpie@explodeLength
\newcount\pgfpie@colorLength
\newcount\pgfpie@sliceLength

\pgfqkeys{/pgfpie}{%
  .search also={/tikz,/pgf},
  explode/.store in=\pgfpie@explode,
  color/.store in=\pgfpie@color,
  radius/.store in=\pgfpie@radius,
  pos/.store in=\pgfpie@pos,
  style/.store in=\pgfpie@style,
  before number/.store in=\pgfpie@beforenumber,
  after number/.code={%
    \def\pgfpie@afternumber{#1}%
    \def\pgfpie@late@afternumber{}%
  },
  text/.store in=\pgfpie@text,
  sum/.code={%
    \def\pgfpie@sum{#1}%
    \pgfpie@ifx\pgfpie@sum\pgfpie@sum@c{%
      \def\pgfpie@late@afternumber{\def\pgfpie@afternumber{\%}}%
    }{%
      \def\pgfpie@late@afternumber{}%
    }%
  },
  rotate/.store in=\pgfpie@rotate,
}

\pgfpie@newif{polar}
\pgfqkeys{/pgfpie}{polar/.is if=pgfpie@polar}

\pgfpie@newif{legend}

\pgfpie@newif{changedirection}
\pgfqkeys{/pgfpie}{change direction/.is if=pgfpie@changedirection}

\pgfpie@newif{square}
\pgfqkeys{/pgfpie}{square/.is if=pgfpie@square}

\pgfpie@newif{cloud}
\pgfqkeys{/pgfpie}{cloud/.is if=pgfpie@cloud}

\pgfpie@newif{scalefont}
\pgfqkeys{/pgfpie}{scale font/.is if=pgfpie@scalefont}
\def\pgfpie@scalefont#1{%
  \pgfpie@ifscalefont{%
    \pgfmathparse{(#1) / (\pgfpie@sum) * 3 + 0.9}%
    \scalefont{\pgfmathresult}%
  }{}%
}

\pgfpie@newif{hidenumber}
\pgfqkeys{/pgfpie}{hide number/.is if=pgfpie@hidenumber}
\def\pgfpie@numbertext#1{%
  \pgfpie@ifhidenumber{}{%
    \pgfpie@beforenumber#1\pgfpie@afternumber
  }%
}

\pgfpie@newif{hidelabel}
\pgfqkeys{/pgfpie}{hide label/.is if=pgfpie@hidelabel}
\def\pgfpie@labeltext#1{\pgfpie@ifhidelabel{}{#1}}

\tikzaddtikzonlycommandshortcutlet{\pie}{\pgfpie@pie}%

\def\pgfpie@pie{%
  \pgfutil@ifnextchar[{\pgfpie@@pie}{\pgfpie@@pie[]}%
}

\def\pgfpie@@pie[#1]#2{%
  \scope[%
    % to be compatible with "babel" lib
    handle active characters in nodes=false,
    % load default parameters
    /pgfpie/.cd,
    explode=0,
    color={blue!60, cyan!60, yellow!60, orange!60, red!60,
      blue!60!cyan!60, cyan!60!yellow!60, red!60!cyan!60,
      red!60!blue!60, orange!60!cyan!60},
    radius=3,
    pos={0,0},
    style={thick},
    before number=,
    after number=,
    text=label,
    sum=100,
    rotate=0,
    change direction=false,
    polar=false,
    square=false,
    cloud=false,
    scale font=false,
    hide number=false,
    hide label=false,
    every pie/.try,%
    % load user's parameters
    #1]

  % add percentage automatically
  \pgfpie@late@afternumber

  % legend or not
  \pgfpie@ifx\pgfpie@text\pgfpie@text@legend{%
    \pgfpie@legendtrue
  }{%
    \pgfpie@legendfalse
  }%

  % handle sum
  \pgfpie@ifx\pgfpie@sum\pgfpie@sum@auto{%
    % sum all input
    \xdef\pgfpie@sum{0}%
    \foreach \pgfpie@p/\pgfpie@t in {#2} {%
      \pgfmathparse{(\pgfpie@sum) + (\pgfpie@p)}%
      \xdef\pgfpie@sum{\pgfmathresult}%
    }%
  }{}%

  % init counters
  \global\pgfpie@explodeLength=0
  \foreach \pgfpie@e in \pgfpie@explode {%
    \global\advance\pgfpie@explodeLength by 1
  }%

  \global\pgfpie@colorLength=0
  \foreach \pgfpie@c in \pgfpie@color {%
    \global\advance\pgfpie@colorLength by 1
  }%
  
  \pgfmathsetlength{\pgfpie@angleEnd}{0}%

  \global\pgfpie@sliceLength=0
  \foreach \pgfpie@p/\pgfpie@e in {#2} {%
    \global\advance\pgfpie@sliceLength by 1
  }%

  \pgfpie@ifsquare{%
    \pgfpie@pie@square{#2}%
    }{\pgfpie@ifcloud{\pgfpie@pie@cloud{#2}%
      }{\pgfpie@pie@circle{#2}}}

  % legend
  \pgfpie@ifhidelabel{}{%
    \pgfpie@iflegend{%
      \pgfpie@legend{#2}%
  }{}}%
  \endscope
}

\def\pgfpie@pie@square#1{%
  \pgfmathparse{(\pgfpie@radius)*2}
  \xdef\pgfpie@verticalLength{\pgfmathresult}
  \xdef\pgfpie@horizontalLength{\pgfmathresult}
  \path (\pgfpie@pos) -- ++({-\pgfpie@radius},{-\pgfpie@radius}) coordinate (pgfpie@start);
  \pgfmathparse{(\pgfpie@verticalLength) * (\pgfpie@horizontalLength) / (\pgfpie@sum)}
  \let\pgfpie@squareUnit\pgfmathresult

  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    \pgfpie@findColor{\pgfpie@i}

    \pgfpie@ifdim{\pgfpie@verticalLength cm}{>}{\pgfpie@horizontalLength cm}{%
      \pgfmathparse{(\pgfpie@p) * (\pgfpie@squareUnit) / (\pgfpie@horizontalLength)}
      \let\pgfpie@height\pgfmathresult
      
      \pgfpie@square{pgfpie@start}{\pgfpie@horizontalLength,\pgfpie@height}
      {\pgfpie@p}
      {\pgfpie@thecolor}
      {\pgfpie@t}
      %label
      \pgfpie@iflegend{}{%
        \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
          \pgfpie@ifhidelabel{}{%
            \path (pgfpie@start) -- ++({\pgfpie@horizontalLength},{\pgfpie@height*0.5})
            node[inner sep=0, \pgfpie@text={0:{\pgfpie@t}}]{};
          }%
        }%
      }%

      \pgfmathparse{\pgfpie@verticalLength - \pgfpie@height}
      \xdef\pgfpie@verticalLength{\pgfmathresult}
      \path (pgfpie@start) -- ++(0, \pgfpie@height) coordinate (pgfpie@start);
    }{%
      \pgfmathparse{(\pgfpie@p) * (\pgfpie@squareUnit) / (\pgfpie@verticalLength)}%
      \let\pgfpie@width\pgfmathresult

      \pgfpie@square{pgfpie@start}{\pgfpie@width,\pgfpie@verticalLength}
      {\pgfpie@p}
      {\pgfpie@thecolor}
      {\pgfpie@t}
      %label
      \pgfpie@iflegend{}{%
        \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
          \pgfpie@ifhidelabel{}{%
            \path (pgfpie@start) -- ++({\pgfpie@width*0.5},{\pgfpie@verticalLength})
            node[inner sep=0, \pgfpie@text={90:{\pgfpie@t}}]{};
          }%
        }%
      }%

      \pgfmathparse{(\pgfpie@horizontalLength) - (\pgfpie@width)}%
      \xdef\pgfpie@horizontalLength{\pgfmathresult}%
      \path (pgfpie@start) -- ++({\pgfpie@width},0) coordinate (pgfpie@start);
    }%
  }%
}

\def\pgfpie@pie@cloud#1{%
  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    % find explode
    \pgfpie@findExplode{\pgfpie@i}
    \def\pgfpie@cloudGap{(\pgfpie@theexplode) + 0.1}
    \pgfmathparse{sqrt((\pgfpie@p) / (\pgfpie@sum)) * (\pgfpie@radius)}
    \let\pgfpie@cloudR\pgfmathresult
    \pgfpie@ifnum{\pgfpie@i}{=}{0}{%
      % first cloud
      \coordinate (pgfpie@O) at (\pgfpie@pos);
      \xdef\pgfpie@cloudRone{\pgfpie@cloudR}
      \xdef\pgfpie@cloudExtendDir{180+(\pgfpie@rotate)}
    }{\pgfpie@ifnum{\pgfpie@i}{=}{1}{%
      % second cloud
      \xdef\pgfpie@cloudRtwo{\pgfpie@cloudR}
      \xdef\pgfpie@cloudExtendDir{45+(\pgfpie@rotate)}
      \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudRtwo)}) coordinate (pgfpie@O);
    }{%
      % next cloud
      \pgfmathparse{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudRtwo)}
      \let\pgfpie@la\pgfmathresult
      \pgfmathparse{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudR)}
      \let\pgfpie@lb\pgfmathresult
      \pgfmathparse{(\pgfpie@cloudRtwo)+(\pgfpie@cloudGap)+(\pgfpie@cloudR)}
      \let\pgfpie@lc\pgfmathresult
      \pgfmathparse{(\pgfpie@la)^2+(\pgfpie@lc)^2-(\pgfpie@lb)^2}
      \let\pgfpie@tmp\pgfmathresult
      \pgfmathparse{180 - acos((\pgfpie@tmp) / 2 / (\pgfpie@la) / (\pgfpie@lc))}
      \let\pgfpie@cloudRot\pgfmathresult
      \pgfpie@ifodd{\pgfpie@i}{%
        \pgfmathparse{-(\pgfpie@cloudRot)}
        \let\pgfpie@cloudRot\pgfmathresult
      }{}%
      \pgfmathparse{(\pgfpie@cloudExtendDir) - (\pgfpie@cloudRot)}
      \xdef\pgfpie@cloudExtendDir{\pgfmathresult}
      \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{\pgfpie@lc}) coordinate (pgfpie@O);
      \xdef\pgfpie@cloudRone{\pgfpie@cloudRtwo}
      \xdef\pgfpie@cloudRtwo{\pgfpie@cloudR}
    }}%

    % find color
    \pgfpie@findColor{\pgfpie@i}

    \pgfpie@cloud{pgfpie@O}{\pgfpie@cloudR}{\pgfpie@p}
    {\pgfpie@thecolor}{\pgfpie@style}{\pgfpie@t}

    % label
    \pgfpie@iflegend{}{%
      \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
        \pgfpie@ifhidelabel{}{%
          \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{\pgfpie@cloudR})
          node[inner sep=0, \pgfpie@text={\pgfpie@cloudExtendDir:{\pgfpie@t}}] {};
        }%
      }%
    }%
  }%
}

\def\pgfpie@pie@circle#1{%
  \pgfpie@ifpolar{%
    \xdef\pgfpie@maxValue{0}
    \foreach \pgfpie@p/\pgfpie@e in {#1} {
      \pgfmathparse{\pgfpie@p}%
      \pgfpie@ifdim{\pgfpie@maxValue pt}{<}{\pgfmathresult pt}{%
        \xdef\pgfpie@maxValue{\pgfpie@p}
      }{}%
    }
    \pgfmathparse{(\pgfpie@sum) / \the\pgfpie@sliceLength}
    \xdef\pgfpie@polarangle{\pgfmathresult}
    \pgfmathparse{(\pgfpie@radius) / sqrt(\pgfpie@maxValue)}
    \xdef\pgfpie@polarRadiusUnit{\pgfmathresult}
  }{%
    \xdef\pgfpie@theradius{\pgfpie@radius}%
  }

  \pgfpie@ifchangedirection{%
    \pgfmathsetlength{\pgfpie@angleEnd}{\pgfpie@sum}
  }{}%
  \xdef\pgfpie@angleBegin{\the\pgfpie@angleEnd}
  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    \pgfmathsetlength{\pgfpie@angleEnd}{\pgfpie@angleBegin}
    \pgfpie@ifpolar{%
      % Polar area diagram
      \pgfmathaddtolength{\pgfpie@angleEnd}{\pgfpie@polarangle}
      \pgfmathparse{sqrt(\pgfpie@p) * (\pgfpie@polarRadiusUnit)}
      \xdef\pgfpie@theradius{\pgfmathresult}
    }{%
      % normal pie
      \pgfpie@ifchangedirection{%
        \pgfmathaddtolength{\pgfpie@angleEnd}{-(\pgfpie@p)}
      }{%
        \pgfmathaddtolength{\pgfpie@angleEnd}{\pgfpie@p}
      }%
    }%

    % find explode
    \pgfpie@findExplode{\pgfpie@i}

    % find color
    \pgfpie@findColor{\pgfpie@i}
    \pgfpie@slice{(\pgfpie@angleBegin)/(\pgfpie@sum)*360+(\pgfpie@rotate)}
    {\the\pgfpie@angleEnd/(\pgfpie@sum)*360+(\pgfpie@rotate)}
    {\pgfpie@p}
    {\pgfpie@t}
    {\pgfpie@theexplode}
    {\pgfpie@thecolor}
    {\pgfpie@theradius}
    {\pgfpie@pos}
    \xdef\pgfpie@angleBegin{\the\pgfpie@angleEnd}
  }
}

\def\pgfpie@legend#1{%
  \coordinate[xshift=0.8cm,
  yshift={(\the\pgfpie@sliceLength*0.5+1)*0.5cm}] (pgfpie@legendpos) at
  (current bounding box.east);

  \scope[node distance=0.5cm]
    \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
    {
      \pgfpie@findColor{\pgfpie@i}
      \node[draw, fill={\pgfpie@thecolor}, \pgfpie@style, below of={pgfpie@legendpos}, label={0:{\pgfpie@t}}] (pgfpie@legendpos) {};
    }
  \endscope
}

